Gender Bias in Transformer Models: A comprehensive survey

Gender bias in artificial intelligence (AI) has emerged as a pressing concern with profound implications for individuals' lives. This paper presents a comprehensive survey that explores gender bias in Transformer models from a linguistic perspective. While the existence of gender bias in language models has been acknowledged in previous studies, there remains a lack of consensus on how to effectively measure and evaluate this bias. Our survey critically examines the existing literature on gender bias in Transformers, shedding light on the diverse methodologies and metrics employed to assess bias. Several limitations in current approaches to measuring gender bias in Transformers are identified, encompassing the utilization of incomplete or flawed metrics, inadequate dataset sizes, and a dearth of standardization in evaluation methods. Furthermore, our survey delves into the potential ramifications of gender bias in Transformers for downstream applications, including dialogue systems and machine translation. We underscore the importance of fostering equity and fairness in these systems by emphasizing the need for heightened awareness and accountability in developing and deploying language technologies. This paper serves as a comprehensive overview of gender bias in Transformer models, providing novel insights and offering valuable directions for future research in this critical domain.

==> Add.tex <==
 \centering Silva et al. \cite{silva2021towards} &
    \centering WEAT, sequence likelihood, and pronoun ranking &
    \centering WEAT scores as a Loss Regularizer \tabularnewline
    \hline

    \centering Joniak et al. \cite{joniak2022gender} &
    \centering SEAT and stereotype score (SS) &
    \centering Movement Pruning \tabularnewline
    \hline

    \centering Robinson et al. \cite{robinson2021assessing} &
    \centering Stereoset Bias Assessment Tool &
    \centering $\textcolor{red}{\times}$ \tabularnewline
    \hline

    \centering \cite{bao2019transfer} &
    \centering Multi-Class Logarithmic Loss &
    \centering Transfer Learning \tabularnewline
    \hline

    \centering \cite{vig2020investigating} &
    \centering Casual Meditation Theory &
    \centering $\textcolor{red}{\times}$ \tabularnewline
    \hline

    \centering \cite{bhardwaj2021investigating} &
    \centering Self Assumption &
    \centering MLP Regression \tabularnewline
    \hline

    \centering \cite{basta2020towards} &
    \centering BLEU Score, Translation Accuracy, F1 Score &
    \centering Contextual Addition \tabularnewline
    \hline

    \centering \cite{bartl2020unmasking} &
    \centering Template-based corpus in English and German &
    \centering Counterfactual Data Substitution \tabularnewline
    \hline

    \centering \cite{kaneko2022gender} &
    \centering Multilingual Bias Evaluation (MBE) score &
    \centering Manual Dataset Creation \tabularnewline
    \hline

    \centering \cite{de2021stereotype} &
    \centering Skew and Stereotype &
    \centering Optimization using an augmented dataset \tabularnewline
    \hline

    \centering \cite{fatemi2021improving} &
    \centering 2nd Phase Training &
    \centering GEEP (Gender Equality Prompt) \tabularnewline
    \hline
